Overfitting or Underfitting? Understand Robustness Drop in Adversarial Training

Our goal is to understand why the robustness drops after conducting adversarial training for too long. Although this phenomenon is commonly explained as overfitting, our analysis suggest that its primary cause is perturbation underfitting. We observe that after training for too long, FGSM-generated perturbations deteriorate into random noise. Intuitively, since no parameter updates are made to strengthen the perturbation generator, once this process collapses, it could be trapped in such local optima. Also, sophisticating this process could mostly avoid the robustness drop, which supports that this phenomenon is caused by underfitting instead of overfitting. In the light of our analyses, we propose APART, an adaptive adversarial training framework, which parameterizes perturbation generation and progressively strengthens them. Shielding perturbations from underfitting unleashes the potential of our framework. In our experiments, APART provides comparable or even better robustness than PGD-10, with only about 1/4 of its computational cost.

==> math_commands.tex <==
%-----------------------------------------------------------------%
%
% The latex macro of the SMiLe group.
%                                       by Han Liu
%
%-----------------------------------------------------------------%

\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{amsthm}
\RequirePackage{bm} 
\RequirePackage{url}
\usepackage{multirow}
%\usepackage{natbib}
\usepackage{graphicx}
%\usepackage{subfigure}
\usepackage{makecell}
\usepackage{booktabs}
\usepackage{array}
\usepackage{url}
%\usepackage{algorithm}
%\usepackage{algorithmic}
\usepackage{dsfont}

\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\let\hat\widehat
\let\tilde\widetilde
\let\check\widecheck
\def\given{{\,|\,}}
\def\ds{\displaystyle}
\newcommand\wtilde{\stackrel{\sim}{\smash{\mathcal{W}}\rule{0pt}{1.1ex}}}

%----- bold fonts -----%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bbb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}
\newcommand{\mub}{\mathbf{\mu}}

\newcommand{\ba}{\bm{a}}
\newcommand{\bb}{\bm{b}}
\newcommand{\bc}{\bm{c}}
\newcommand{\bd}{\bm{d}}
\newcommand{\be}{\bm{e}}
\newcommand{\bbf}{\bm{f}}
\newcommand{\bg}{\bm{g}}
\newcommand{\bh}{\bm{h}}
\newcommand{\bi}{\bmf{i}}
\newcommand{\bj}{\bm{j}}
\newcommand{\bk}{\bm{k}}
\newcommand{\bl}{\bm{l}}
\newcommand{\bbm}{\bm{m}}
\newcommand{\bn}{\bm{n}}
\newcommand{\bo}{\bm{o}}
\newcommand{\bp}{\bm{p}}
\newcommand{\bq}{\bm{q}}
\newcommand{\br}{\bm{r}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bt}{\bm{t}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bx}{\bm{x}}
\newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}




\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\bA}{\bm{A}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bD}{\bm{D}}
\newcommand{\bE}{\bm{E}}
\newcommand{\bF}{\bm{F}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bJ}{\bm{J}}
\newcommand{\bK}{\bm{K}}
\newcommand{\bL}{\bm{L}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bT}{\bm{T}}
\newcommand{\bU}{\bm{U}}
\newcommand{\bV}{\bm{V}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bX}{\bm{X}}
\newcommand{\bY}{\bm{Y}}
\newcommand{\bZ}{\bm{Z}}


%----- calligraphic fonts -----%

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cT}{{\mathcal{T}}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}




%----- blackboard bold fonts-----%

\newcommand{\CC}{\mathbb{C}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\OOmega}{\mathbb{\Omega}}




%----- bold greek fonts -----%

\newcommand{\balpha}{\bm{\alpha}}
\newcommand{\bbeta}{\bm{\beta}}
\newcommand{\bgamma}{\bm{\gamma}}
\newcommand{\bepsilon}{\bm{\epsilon}}
\newcommand{\bvarepsilon}{\bm{\varepsilon}}
\newcommand{\bzeta}{\bm{\zeta}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\bvartheta}{\bm{\vartheta}}
\newcommand{\bkappa}{\bm{\kappa}}
\newcommand{\blambda}{\bm{\lambda}}
\newcommand{\bmu}{\bm{\mu}}
\newcommand{\bnu}{\bm{\nu}}
\newcommand{\bxi}{\bm{\xi}}
\newcommand{\bpi}{\bm{\pi}}
\newcommand{\bvarpi}{\bm{\varpi}}
\newcommand{\brho}{\bm{\varrho}}
\newcommand{\bsigma}{\bm{\sigma}}
\newcommand{\bvarsigma}{\bm{\varsigma}}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\bupsilon}{\bm{\upsilon}}
\newcommand{\bphi}{\bm{\phi}}
\newcommand{\bvarphi}{\bm{\varphi}}
\newcommand{\bchi}{\bm{\chi}}
\newcommand{\bpsi}{\bm{\psi}}
\newcommand{\bomega}{\bm{\omega}}

\newcommand{\bGamma}{\bm{\Gamma}}
\newcommand{\bDelta}{\bm{\Delta}}
\newcommand{\bTheta}{\bm{\Theta}}
\newcommand{\bLambda}{\bm{\Lambda}}
\newcommand{\bXi}{\bm{\Xi}}
\newcommand{\bPi}{\bm{\Pi}}
\newcommand{\bSigma}{\bm{\Sigma}}
\newcommand{\bUpsilon}{\bm{\Upsilon}}
\newcommand{\bPhi}{\bm{\Phi}}
\newcommand{\bPsi}{\bm{\Psi}}
\newcommand{\bOmega}{\bm{\Omega}}


%----- Some standard definitions -----%

\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\minimize}{\mathop{\mathrm{minimize}}}

\newcommand{\sign}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}

\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator{\Var}{{\rm Var}}
\DeclareMathOperator{\Cor}{\rm Corr}
\DeclareMathOperator{\Cov}{\rm Cov}
\DeclareMathOperator{\ind}{\mathds{1}}  % Indicator
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}  
                                                        
\newcommand*{\zero}{{\bm 0}}
\newcommand*{\one}{{\bm 1}}

\newcommand{\diag}{{\rm diag}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%% Norms

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\bignorm}[1]{\bigg|\bigg|#1\bigg|\bigg|}
\newcommand{\opnorm}[2]{| \! | \! | #1 | \! | \! |_{{#2}}}

%%%%% Dot product
\newcommand{\dotp}[2]{\langle{#1},{#2}\rangle}

%%%%  brackets
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}

%%%%%%%%%  Other commands

\newcommand{\mcomment}[1]{\marginpar{\tiny{#1}}}
\newcommand{\fcomment}[1]{\footnote{\tiny{#1}}}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\ud}{{\,\mathrm{d}}}


%%%%%%%%  amsmath %%%%%%%%%%
% Bourbaki style
\newtheoremstyle{plain} % name 
    {1.5}                    % Space above
    {1.5}                    % Space below
    {\normalfont}                   % Body font
    {}                           % Indent amount
    {\scshape}                   % Theorem head font
    {.~---}                          % Punctuation after theorem head
    {.5em}                       % Space after theorem head
    {}  % Theorem head spec (can be left empty, meaning ‘normal’)

\theoremstyle{plain}

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi
\ifx\example\undefined
\newtheorem{example}{Example}
\fi
\ifx\property\undefined
\newtheorem{property}{Property}
\fi
\ifx\lemma\undefined
\newtheorem{lemma}{Lemma}
\fi
\ifx\proposition\undefined
\newtheorem{proposition}{Proposition}
\fi
\ifx\remark\undefined
\newtheorem{remark}{Remark}
\fi
\ifx\corollary\undefined
\newtheorem{corollary}{Corollary}
\fi
\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi
\ifx\conjecture\undefined
\newtheorem{conjecture}{Conjecture}
\fi
\ifx\fact\undefined
\newtheorem{fact}{Fact}
\fi
\ifx\claim\undefined
\newtheorem{claim}{Claim}
\fi
\ifx\assumption\undefined
\newtheorem{assumption}{Assumption}
\fi
\ifx\condition\undefined
\newtheorem{condition}{Condition}
\fi

\newtheoremstyle{anothertheoremstyle} % name
    {\topsep}                    % Space above
    {\topsep}                    % Space below
    {\normalfont}                   % Body font
    {}                           % Indent amount
    {\bfseries}                   % Theorem head font
    {.}                          % Punctuation after theorem head
    {.5em}                       % Space after theorem head
    {\thmname{#1} \thmnumber{#2} \normalfont{#3}}  % Theorem head spec (can be left empty, meaning ‘normal’)
\makeatletter
\newcommand{\raisemath}[1]{\mathpalette{\raisem@th{#1}}}
\newcommand{\raisem@th}[3]{\raisebox{#1}{$#2#3$}}
\makeatother

\let\oldabstract\abstract
\let\oldendabstract\endabstract
\makeatletter
\renewenvironment{abstract}
{\renewenvironment{quotation}%
               {\list{}{\addtolength{\leftmargin}{-0.5em} % change this value to add or remove length to the the default
                       \listparindent 3em%
                        \itemindent    \listparindent%
                        \rightmargin   \leftmargin%
                        \parsep        \z@ \@plus\p@}%
                \item\relax}%
               {\endlist}%
\oldabstract}
{\oldendabstract}
\makeatother


==> src/exp_old.tex <==
\section{Experiments}
\label{sec:exp}

% In this section, we apply our proposed \our training framework to multiple neural architectures on multiple data sets. 
% By evaluating the robustness and efficiency, we show that \our is able to achieve a better performance than other popular adversarial training methods. 
% To understand the contributions of each part in \our, we conduct an ablation study.


\subsection{Experimental Settings}

\smallsection{Datasets}
We conduct experiments on the CIFAR-10, CIFAR-100 datasets~\citep{Krizhevsky2009LearningML} and ImageNet~\citep{krizhevsky2012imagenet}.

\smallsection{Neural Architectures}
To show the generality of our \our framework, we conduct experiments with Pre-Act ResNet~\citep{he2016identity} and WideResNet~\citep{Zagoruyko2016WideRN}.
Specifically, we use Pre-Act ResNet18 and WideResNet34-10 on CIFAR-10, Pre-Act ResNet18 on CIFAR-100, and ResNet50~\citep{he2016deep} on ImageNet. 
% We evaluate the robustness on CIFAR-10 with Pre-Act ResNet18 and WideResNet34-10. And we use Pre-Act ResNet18 to evaluate the performance on CIFAR100. And ResNet50~\citep{he2016deep} is used for ImageNet.

\smallsection{Data Augmentation}
% \todo{add citations about the source of this config. }
For CIFAR-10 and CIFAR-100, We apply random flipping as a data augmentation procedure and take a random crop with $32 \times 32$ from images padded by $4$ pixels on each side~\citep{Lee2015DeeplySupervisedN}. 
For ImageNet, we divide the training into three phases, where phase 1 and 2 use images resized to 160 and 352 pixels and the third phase uses the whole images~\citep{Wong2020FastIB}. 


\smallsection{Optimizer}
% \todo{add citations about the source of this config. }
For all experiments on CIFAR-10 and CIFAR-100, we use SGD solver~\citep{Robbins2007ASA} with momentum of 0.9 and cyclic learning rate decay.
Cyclic learning rate scheduler~\citep{Smith2017CyclicalLR} is proposed to help convergence of neural networks and reduce the number of learning rate trials. 
Specificcally, the learning rate starts from zero, reaches to the maximum learning rates and decreases to zero. 
% The scheduler can help the model reach to the baseline much faster within tens of epochs.
For ImageNet, we also use cyclic learning rate scheduler and the scheduler is decayed further by a factor of 10 in the second and third phases~\citep{Wong2020FastIB}.


\smallsection{Attacks for Robustness Evaluation}
We adopt PGD-20~\citep{Madry2017TowardsDL}, Gaussian random noise, and C\&W~\citep{Carlini2017TowardsET} as the attack method for evaluation. For PGD attack, we apply $\epsilon=8/255$ on CIFAR-10 and CIFAR-100, $\epsilon=2/255$ on ImageNet.

\smallsection{Infrastructure}
Our experiments are conducted with NVIDIA Quadro RTX 8000 GPUs, and mixed-precision arithmetic~\citep{Micikevicius2018MixedPT} is further adopted to accelerate model training. 
The training speed of our method or baselines is evaluated on an idle GPU. 
% To accelerate adversarial training and reduce memory utilization, we adopt mixed-precision arithmetic~\citep{Micikevicius2018MixedPT}
% Mixed-precision arithmetic~\citep{Micikevicius2018MixedPT} is further adopted to accelerate model training. 




\subsection{Compared Methods}
We select four state-of-the-art adversarial training methods for comparison. 
To ensure a fair comparison on efficiency, we report accuracy and training time based on our experiments on CIFAR-10 and CIFAR-100. 
As to ImageNet, we directly refer to the number reported in the original papers.
\begin{itemize}[nosep, leftmargin=*]
    \item \textbf{PGD-K}\citep{Madry2017TowardsDL} is a classical, sophisticated adversarial training method. PGD is an iterative version of FGSM \todo{i dont think this is true, as it does not take sign?}\zichao{but in each iteration, it gets the sign of gradient}with uniform random noise as initialization and K is the number of iterations.
    % Here we use  PGD-10 with step size $\alpha = 2/255$ and $\epsilon = 8/255$. For all baselines and our methods, the $\epsilon = 8/255$.  %\todo{epsilon should be same for all methods?}.
    \item \textbf{Free-m}~\citep{Shafahi2019AdversarialTF} updates both the model parameters and image perturbations with one simultaneous backward pass instead of separate computations by training on the same minibatch $m$ times in a row. Here we set $m = 8$
    % , rather than using separate gradient computations for each update step. 
    \item \textbf{ATTA-K}~\citep{Zheng2019EfficientAT} uses the adversarial examples from neighboring epochs. K is the number of iterations and denotes the strength of attack. 
    \item \textbf{F+FGSM}~\citep{Wong2020FastIB} uses a large step size and random initialization to improve the performance of FGSM to be comparable to that of PGD-10.
    % F+FGSM is the state-of-the-art considering both robustness and efficiency compared to the other three.

\end{itemize}

% We denote our training framework as \our. \our(w/o l.w.n.) denotes that we do not use the layer-wise noise in our framework and \our(w/o p.) refers that we only the gradient information of the current epoch without information from previous epochs

\subsection{Performance Comparison}

\smallsection{CIFAR-10}
% To compare the efficiency fairly, we run for 30 epochs for each method with cyclic learning rate schedule. \todo{move the number of epochs to the dataset setting}.
% We do experiments on Pre-Act ResNet18~\citep{he2016identity}, WideResNet34~\citep{Zagoruyko2016WideRN} and summarize the results in Table~\ref{table:preact} and Table~\ref{table:cifar10, wide}. 
We summarize the model performance in Table~\ref{table:preact} and Table~\ref{table:cifar10, wide}. 
% As shown in Table~\ref{table:preact}, our method improves adversarial accuracy by 1.67\% with 4.6 times training efficiency.
For Pre-Act ResNet18, \our improves adversarial accuracy over 
PGD-10 with 4.6 times acceleration. 
For example, as PGD-10 leads to a $47.43\%$ accuracy under the PGD-20 attack, \our achieves a $49.26\%$ accuracy. 
Among all methods, \our achieves the highest adversarial accuracy under PGD-20, Gaussian random noise and C\&W attack, with a satisfying performance on clean images. 
% As for WideResNet34-10, \our still achieves similar acceleration compared to PGD-10 and has better robustness than other four methods with only a little drop in clean accuracy.
% \todo{is it WideResNet34? or 34-10?}
Similar pattern is observed for WideResNet34-10, \our outperforms PGD-10 under various of attacks with a 4.2 times speedup, at the cost of some clean accuracy. 

\smallsection{CIFAR-100}
% \todo{how many epochs?}
% Table~\ref{table:cifar100} shows the results for training an CIFAR-100 classifier with \our. 
% With a 100 classes task, \our has a 2.39\% higher adversarial accuracy than PGD-10 and improves the robustness performance by 2.19\% comapred to Fast.
We summarize model performances in Table~\ref{table:cifar100}. 
Similar to CIFAR-10, \our is not only faster than PGD-10 (4.6 times faster), but also has more robustness (more than 1\% absolute accuracy). 
It is worth mentioning that, \our achieves the highest performance on corrupted images, 2rd highest performance on clean images, and 2rd fastest training speed. 

\smallsection{ImageNet}
% Table~\ref{table:ImageNet} shows the results for training an ImageNet classifier with $\ell_{\infty}(\epsilon=2/255)$. 
% \todo{what is the epsilon for CIFAR-10 and CIFAR-100?, move this information to Sec. 5.1, Attacks for Robustness Evaluation.}
\zichao{I didn't reproduce the imagenet experiment of other methods, so we cite the time cost in their paper directly?}
We summarize model performances in Table~\ref{table:ImageNet}.
Among all compared methods, ATTA-2 reaches the highest accuracy under PGD-10 attack at the cost of highest computation costs. 
\our achieves a similar performance with ATTA-2, but 

\begin{table}[t]
  \caption{Model Performance of Pre-Act ResNet18 on CIFAR-10.}
  \label{table:preact}
  \centering
%   \small
  \begin{tabular}{llllll}
    \toprule
    Training Methods & Clean Data & PGD-20 Attack & C\&W Attack & Gaussian Noise & Time(s)\\
    \midrule
    ATTA-10 & 82.10\% & 49.03\% & 58.30\% & 73.10\% & 140\\
    PGD-10 & 82.05\% &  47.43\% & 56.55\% & 72.33\% & 133\\
    Free(m=8) & 81.64\% & 47.37\% & 56.10\% & 72.56\% &62\\
    F+FGSM & {83.81\%} & 46.06\% & 55.34\% & 72.25\% & {20}\\
    \our & 82.45\% & {49.30\%} & {58.50\%} & {73.18\%} & 29\\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[t]
  \caption{Model Performance of WideResNet34-10 on CIFAR-10.}
  \label{table:cifar10, wide}
  \centering
%   \small
  \begin{tabular}{llllll}
    \toprule
    Training Methods & Clean Data &  PGD-20 Attack  & C\&W Attack & Gaussian Noise & Time(s) \\
    \midrule
    ATTA-10 & 83.80\% & 54.33\% &  59.11\% & 77.05\% & 706 \\
    PGD-10 & 86.43\% & 47.12\% & 56.45\% & 75.70\% &680 \\
    Free(m=8) & 85.54\% & 47.68\% & 56.31\% & 75.98\% &252 \\
    F+FGSM & 85.10\% & 46.37\% &  56.21\% & 75.10\% & 122 \\
    \our & 84.75\%  & 51.10\% &  58.50\% & 76.50\% & 162\\

    \bottomrule
  \end{tabular}
\end{table}

% \subsection{Performance on other datasets}

\begin{table}[t]
%   \caption{Robustness Evaluation. We conduct experiments on CIFAR-100 with Pre-Act ResNet20. The performance of our method outperforms that of PGD-10 and other adversarial training methods.}
  \caption{Model Performance of Pre-Act ResNet20 on CIFAR-100.}
  \label{table:cifar100}
  \centering
  \begin{tabular}{llllll}
    \toprule
    % \multicolumn{2}{c}{Part}                   \\
    Training Methods & Clean Data & PGD-20 Attack & C\&W Attack & Gaussian Noise & Time (min)\\
    \midrule
    ATTA-10 & 56.20\% & 25.60\% & 30.75\% & 42.10\% & 140\\
    PGD-10 & 55.14\% &  25.61\%  &30.65\%  &  42.41\% & 133\\
    Free(m=8) & 55.13\% & 25.88\% & 30.55\% &42.15\% &62\\
    F+FGSM & 57.95\% & 25.31\% & 30.06\% & 42.03\%& {20} \\
    \our & 57.10\% & {27.10}\% & 32.36\% & 43.30\%& 29\\
    
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}[t]
  \caption{Model Performance of ResNet50 on CIFAR-100.}
  \label{table:ImageNet}
  \centering
  \begin{tabular}{lll}
    \toprule
    % \multicolumn{2}{c}{Part}                   \\
    Training Methods & Clean Data & PGD-10 Attack \\
    \midrule
    ATTA-2~\citep{Zheng2019EfficientAT} & 60.70\% & 44.57\% \\
    Free(m=4)~\citep{Shafahi2019AdversarialTF} & 64.44\% & 43.52\%  \\
    F+FGSM~\citep{Wong2020FastIB} & 60.90\% & 43.46\% \\
    \our & 60.52\% & 44.50\% \\
    
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Balance between Clean Accuracy and Accuracy under PGD-20 Attack}
We conduct experiments to illustrate the robustness of different methods with different $\epsilon$ under PGd-20 attack. Figure~\ref{fig:diff_eps} shows that \our has better performance than other four methods with different $\epsilon$.

\subsection{Ablation Studies}
To compare the contributions of each part of \our, we use \our to train the model without various part of our method. 
We also try to only use the gradients from previous epochs. 
As our method uses adaptive parameter to control the step size of layer-wise attack, we shows the role of perturbations from various layer during adversarial training. Besides, we explore the robustness performance of various methods with various $\epsilon$.


As shown in Table ~\ref{table:part}, without layer-wise noise, there will be a 2.75\% drop and the drop is 1.8\% without using the gradients from previous epochs compared to the full \our. 
Table~\ref{table:part} also shows that , while gradients from previous epochs help improve the robustness, only using them cannot make models robust.
\begin{table}[t]
  \caption{Contributions of each part of \our. We conduct experiments on the CIFAR-10 dataset with Pre-Act ResNet-20.}
  \vspace{2mm}
  \label{table:part}
  \centering
  \begin{tabular}{lll}
    \toprule
    Training Methods & Clean Data & PGD-20 Attack \\
    \midrule
    \our & 82.45\% & 49.30\% \\ 
    \our(w/o layer-wise perturbation) & 83.30\% & 46.35\%\\
    \our(w/o perturbation initialization) & 82.50\% & 47.30 \%\\
    Previous gradients only & 93.50\% & 0.00\% \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Changing Trend of Step-Sizes}
% \smallsection{Growth of the step size of perturbations from layers}
As mentioned in previous section, \our uses adaptive step size for the perturbations added to the intermediate features of each block. 
All step sizes start from the same value and are updated with parameters of network during training.
Figure ~\ref{fig:eps} shows that the step size of the perturbation of the first convolutional layer is much higher than that of other layers. 


% \begin{figure}[t]
% \vskip 0.2in
% \begin{center}

% \centerline{\includegraphics[width=0.7\columnwidth, scale=2]{figures/eps.pdf}}
% \caption{Growth of step sizes}
% \label{figure:eps}

% \end{center}
% \vskip -0.2in
% \end{figure}


% \zichao{if I should use early stopping for fast method or use the current fig to show its drawbacks}

% \begin{figure}[t]
% \vskip 0.2in
% \begin{center}

% \centerline{\includegraphics[width=0.7\columnwidth, scale=2]{figures/diff_eps.pdf}}
% \caption{Growth of step sizes}
% \label{figure:diff_eps}

% \end{center}
% \vskip -0.2in
% \end{figure}

\begin{figure}[t]
\centering
\begin{minipage}[t]{0.6\textwidth}
\centering
\includegraphics[height=1.75in]{figures/eps.pdf}
\caption{Growth of step sizes\zichao{why tuned 0.6 t0 0.5? if 0.5, we cannot see the legend}}
\label{fig:eps}
\end{minipage}%
\begin{minipage}[t]{0.4\textwidth}
\centering
\includegraphics[height=1.75in]{figures/diff_eps.pdf}
\caption{Performance with various $\epsilon$ }
\label{fig:diff_eps}
\end{minipage}
\end{figure}

==> src/overfit_old.tex <==

\section{The Mechanism of The Robustness Drop: A Perturbation Strength Perspective}

% After conducting adversarial training for too long, it has been observed that the model robustness drops significantly. 
Robustness drop has been widely observed after conducting adversarial training for too long.
For example, in Figures~\ref{fig:learning_curve}, the training objective of PGD-10 keeps decreasing, while the model robustness starts to drop after the 20th epoch. 
Remarkably, stopping the FGSM training at the 21st epoch would yield a 0\% test robustness accuracy under the PGD-20 attack (as in Figure~\ref{fig:fgsm_analysis}). 
Because of the performance gap between the robustness on the training set and the test set, this phenomenon has been long-regarded as overfitting.
However, its underlying mechanism remains mysterious. 
Here, we conduct systematic analyses to pursue its underpinnings. 

\begin{figure*}[t]
  \centering
    \subfigure[Training Robustness Accuracy]{\includegraphics[width=0.45\textwidth]{figures/train.pdf}} 
	\subfigure[Test Robustness Accuracy (PGD-20 attack)]{\includegraphics[width=0.45\textwidth]{figures/test.pdf}} \\

  \caption{
  Our proposed \our better resolves the robustness drop issue than PGD-10. \our(F) denotes that we only add noise to the input images.
%   (a) the robust training accuracy; (b) the robust test accuracy under PGD-20 attack.
}
	\label{fig:learning_curve}
\end{figure*}


\subsection{Perturbation Strength Gap}


Comparing the robustness drop of FGSM and PGD, we observe that it leads to a smaller drop by using more complex perturbation generation models. 
Intuitively, since the robustness drop can be alleviated by using more powerful perturbations, the gap between these perturbation generation methods and ideal perturbations are too large. 
To further verify our intuition, we empirically estimate the perturbation strength.
For $\theta_{\mathcal{A}}^{(i)}$ and $f_{\cA}$, we approximate the perfect perturbation with a more powerful attack method $f_{\cB}$ and calculate the gap as $\cG_{\mathcal{A}\to\mathcal{B}}$ in Equation~\ref{eqn:cg_fgsm_pgd10}. 
% To further verify our intuition, we empirically estimate the perturbation strength gap between FGSM and PGD-10 with the $\cG_{\fgsm\to\pgd{10}}$ in Equation~\ref{eqn:cg_fgsm_pgd10}.
% To further verify our intuition, we empirically estimate a gap between adversarial training method $\mathcal{A}$ and $\mathcal{B}$ as $\cG_{\fgsm\to\pgd{10}}$ in Equation~\ref{eqn:cg_fgsm_pgd10}, which approximates the perfect perturbation for $\theta_{\fgsm}^{(i)}$ with the perturbation generated by a more powerful method, PGD-10. 
% $\mathcal{B}$.
% with the gap between perturbations generated by $\mathcal{A}$ and $\mathcal{B}$ as $\cG_{\mathcal{A}\to\mathcal{B}}$ in Equation~\ref{eqn:cg_fgsm_pgd10}, which approximates the perfect perturbation for $\theta_{\mathcal{A}}^{(i)}$ with the perturbation generated by a more powerful method, $\mathcal{B}$. 


% \begin{equation}
% \label{eqn:cg_fgsm_pgd10}
% \cG_{\fgsm\to\pgd{10}} = \gL(\theta^{(i)}_{\fgsm}; \xb+\delta^{(i)}_{\fgsm}, y) - \gL(\theta^{(i)}_{\fgsm};\xb+\delta^{(i)}_{\pgd{10}}, y).
% \end{equation}

\begin{equation}
\label{eqn:cg_fgsm_pgd10}
\cG_{\mathcal{A}\to\mathcal{B}}(\theta^{i}_\mathcal{A}) = \gL(\theta^{(i)}_{\mathcal{A}}; \xb+f_{\mathcal{B}}(\theta^{(i)}_{\mathcal{A}}, \xb, y), y) - \gL(\theta^{(i)}_{\mathcal{A}};\xb+\delta_{\mathcal{A}}, y).
\end{equation}

% \jingbo{
% Please formulate $\cG$ in a more general way by comparing a simple training vs. a more complex training. 
% And then, give a few examples, such as $\cG_{\fgsm\to\pgd{10}}$, $\cG_{\text{our}\to\pgd{10}}$, and $\cG_{\pgd{5}\to\pgd{10}}$. 
% These are used in later discussions or figures.
% }

% \jingbo{We probably want to give a notation to the ``ideal perturbation generation''.  $\cG$ involving this might be impossible to compute, however, we can get its lowerbound by replace the ``ideal'' one by any other complex generation process. This will make the flow more smooth.}


The value of $\cG_{\fgsm\to\pgd{10}}$ is calculated with Pre-Act ResNet18 on the CIFAR10 dataset, and the results are visualized in Figure~\ref{fig:diff_loss}(a). 
It shows that the strength gap is small in the early stage, dramatically explodes at the 21st epoch and keeps a large value since then. 
Since this time point coincides with the time point of the robustness drop, it implies the strength gap to be the reason of the robustness drop. 
We also conduct empirical evaluations for PGD, visualize $\cG_{\pgd{5}\to\pgd{20}}$ in Figure~\ref{fig:diff_loss}(b), and observe a similar phenomenon, \ie, the gap keep increasing during the training. 

% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}

% \centerline{\includegraphics[width=0.5\columnwidth, scale=2]{figures/diff_loss.pdf}}
% \caption{Difference of loss between  PGD-10(~\cite{Madry2017TowardsDL}) examples and FGSM(~\cite{goodfellow2014explaining}) examples generated by robustly trained model with FGSM}
% \label{figure:diff_loss}
% % \includegraphics[]{}
% % \label{icml-historical}
% \end{center}
% \vskip -0.2in
% \end{figure}
\begin{figure*}[t]
  \centering
    \subfigure[$\cG_{\fgsm\to\pgd{10}}(\theta^{(i)}_{\fgsm})$ vs. $\cG_{\text{\our}\to\pgd{10}(\theta^{(i)}_{\text{\our}})}$]{
        \includegraphics[width=0.48\textwidth]{figures/diff_loss.pdf}
    } 
	\subfigure[$\cG_{\pgd{5}\to\pgd{20}}(\theta^{(i)}_{\pgd{5}})$]{\includegraphics[width=0.48\textwidth]{
	    figures/20-5diff.pdf}
	}
  \caption{
  Comparing perturbation generations versus more complex ones using Pre-Act ResNet18 on the CIFAR-10 dataset, we believe that there exists a large gap between the generated perturbations and the ideal perturbations. Our proposed \our is able to close this gap significantly.
%   Left: Difference of loss value between  PGD-10~\citep{Madry2017TowardsDL} examples and FGSM~\citep{goodfellow2014explaining} examples generated by robustly trained model with FGSM; Right: Difference of loss between  PGD-5 examples and PGD-20 examples generated by robustly trained model with PGD-5. 
  }
	\label{fig:diff_loss} 
\end{figure*}


% \subsection{Deterioration of Adversarial Training}
% To further evaluate the strength of generated perturbations, we use a model which is separately trained with PGD-10. 
% Specifically, we visualize $\gL(\theta_{\pgd{10}}; \xb+f_{\fgsm}(\theta_{\fgsm}^{(i)}, \xb, y), y)$ in Figure~\ref{fig:random}(b). 
% The strength of perturbations increases in the early stage, and decreases dramatically later. 
% Intuitively, gradient-guided perturbation generator share similar intuitions with some neural network interpretation methods\todo{add citations}.
% Thus, the generator can benefit from the strength gained in the CNN model, which leads to the more effective perturbations in the early stage.
% In the late stage, the dramatic strength drop also provides evidence supporting the deterioration of FGSM. 



% \jingbo{Is it too late to discuss here? I feel it's a bit redundant. Most of the info have been covered in  intro?) I will suggest to fuse it into the intro and shout ``Deterioration of FGSM'' out.}
% \jingbo{Maybe we can combine this Deterioration of FGSM and PDG together and rename the subsection as ``Deterioration of Adversarial Training''}

% \zichao{I think the deterioration of PGD is not necessary. We already have the perturbation part for PGD }

\subsection{Deterioration of FGSM}
\label{subsec:fgsm_deterioration}


% Here, we conduct empirical evaluations on the strength of FGSM-generated perturbations. 
% Firstly, we visualize perturbations generated by FGSM in Figure~\ref{fig:random}, i.e., $\delta_{\fgsm}^{(i)}$ where $i = 18$ and $i = 30$. 
% While these perturbations mostly resemble random noise after the robustness drop (at the 19 epoch), they are able to surgically alter the image at the 18th epoch. 
% For example, the perturbation generated for the airplane image distinguishes the airplane body and the background, which effectively identifies the airplane-indicating features thus poisoning model outputs. 
% As discussed in ~\citet{Ilyas2019AdversarialEA}, the generated perturbations, although subtle, contain output-indicating information.
% However, this pattern is disappeared after the robustness drop. 
% At the 18th epoch, the perturbations are generated in a random manner. 

To further understand the significant robustness drop of FGSM, we further analyze the strength of FGSM-generated perturbations. 
Specifically, we aim to explore, while the FGSM-generated perturbations resemble random noise at the 30-th epoch, whether these perturbations behave similar to random noise. 
Thus, we test these perturbations, together with random noise, on a model that is separately trained with PGD-10.
We visualize the accuracy curves of $Acc(\theta_{\pgd{10}}, f_{\fgsm}(\theta^{(i)}_{\fgsm}, \cdot))$ and $Acc(\theta^{(i1)}_{\pgd{10}}, f_{\random}(\cdot))$ in Figure~\ref{fig:defense}. 
The strength of perturbations increases in the early stage, and decreases dramatically later to the random noise level. 
% Intuitively, gradient-guided perturbation generator share similar intuitions with some neural network interpretation methods\todo{add citations}.
% Thus, the generator can benefit from the strength gained in the CNN model, which leads to the more effective perturbations in the early stage.
% In the late stage, the dramatic strength drop also provides evidence supporting the deterioration of FGSM. a
Also, this perturbation effectiveness drop happens at the 19 epoch, the same epoch where the significant robustness drop happens, which is another evidence verifying our intuition. 

% \subsection{Alleviating Robustness Drop by Parameterizing Perturbation Generation}

% \jingbo{What are we going to do here? This looks like our method part? Do you want to try the simplest version of \our method and use it as a proof-of-concept?}

We try to further verify the intuition that shielding perturbations from underfitting could alleviate the robustness drop. 
Intuitively, one straightforward way to strengthen perturbations is to parameterize the perturbation generator and update them together with model parameters. 
Specifically, we treat the perturbation initialization for the input (referred as $\omega_\xb$) and the step size (referred as $\alpha$) as parameters of FGSM, and change the objective from Equation~\ref{eq:min} to:
\begin{equation}
\label{eq:max-min}
    \max_{\alpha, \omega} \min_{\theta} \cL(\theta; \xb + f_{\fgsm}(\alpha, \omega_\xb; \theta, \xb, y), y).
\end{equation}
Note that although $f_{\fgsm}(\cdot)$ also includes a process to maximize the objective function, the strength of its generated perturbations is static without updating this process. 
Its training accuracy and test accuracy is visualized in \todo{add visualizations here}.
This not only supports our intuition that the perturbation underfitting contributes a lot to the robustness drop, but motivates us to shield generators by parameterizing and strengthening them with gradient updates.

% \begin{figure}[t]
% \vskip 0.2in
% \begin{center}

% \centerline{\includegraphics[width=0.5\columnwidth, scale=2]{figures/defense.png}}
% \caption{Left: The learning curve for a robustly trained model done by FGSM(~\cite{goodfellow2014explaining}) with $l_\infty$ radius $\epsilon$ = 8/255; Right: The defense curve for a PGD-10(~\cite{Madry2017TowardsDL}) trained model attacked by the examples generated by FGSM(~\cite{goodfellow2014explaining}) from various epochs.}
% \label{fig:defense}
% % \includegraphics[]{}
% % \label{icml-historical}]
% \end{center}
% \vskip -0.2in
% \end{figure}

% \subsection{Deterioration of PGD}
% we also conduct empirical evaluations on the strength of PGD-generated perturbations. We visulize $\gL(\theta_{\pgd{5}}; \xb+f_{\pgd{5}}(\theta_{\pgd{5}}^{(i)}, \xb, y), y)$ and $\gL(\theta_{\pgd{5}}; \xb+f_{\pgd{20}}(\theta_{\pgd{5}}^{(i)}, \xb, y), y)$ in Figure~\ref{fig:diff_loss}(b). As we train for longer time, the difference between the two losses becomes larger. 

% \subsection{Alleviating Robustness Drop by Parameterizing Perturbation Generation}

% \jingbo{What are we going to do here? This looks like our method part? Do you want to try the simplest version of \our method and use it as a proof-of-concept?}

% Intuitively, previous analysis implies the robustness drop is caused by the perturbation underfitting. 
% Here, we further verify our intuition by ... 












